A Model Organism for Studying Unverbalized Evaluation Awareness

Large language models can recognize when they are being evaluated and change their behavior accordingly, undermining the reliability of safety benchmarks. Evaluation awareness (EA) is usually measured by having an LLM judge scan reasoning traces for explicit statements of recognition, but this signal is increasingly unreliable. Recent frontier-model system cards report a drop in verbalized rates between releases, which is indistinguishable from awareness that has gone unverbalized. Interpretability methods could detect such unverbalized evaluation awareness (UEA) in individual interactions, but lack instance-level ground truth. Asking the model alters the input, and dataset labels do not reveal whether it recognized a particular prompt as an evaluation. We address this gap with a model organism. Using synthetic document fine-tuning, SFT, and DPO, we train Qwen3.5-27B to emit a marker (a designated token) in its final response when it recognizes an evaluation, while suppressing the marker and verbalized awareness in its reasoning. The marker largely tracks the evaluation concept as it can be strongly modulated by evaluation framing in the system prompt. When not told whether it is being evaluated, the organism recognizes evaluations from test-question cues, mirroring what its base model often verbalizes. Using the marker as a label, we benchmark linear probes, the Jacobian Lens, and Activation Oracles, built on the base model and blind to the marker. None recovers the label reliably. These results suggest that current interpretability methods are not yet reliable UEA detectors, even when recognition relies on simple cues. Our model organism offers a testbed for improving them.

==> sections/experimental_evaluation.tex <==
\subsection{Experimental Setup}
\sahar{we might save space if we make one section as experimental evaluation with one subsection as setup, if needed}
\label{sec:experiment_setup}
\input{sections/experimental_setup}

\subsection{Results}
\label{sec:results}
\input{sections/results}

==> sections/methods/interpretability.tex <==
\subsubsection{Probes}

We test ten linear probes, built on the base model, to score activations extracted from the model organism. We build two main types of probes, contrastive means and trained.

We first build four directions that are the normalized difference in mean activation between evaluation and deployment prompts, read at the prompt's final token: \textbf{TH-16}, the 16 prompt pairs of \citet{hua2025steering}; \textbf{TH-4}, the four of those pairs they single out; \textbf{Anth}, the single contrastive pair of \citet{anthropic2026opus47}; and \textbf{E/NE}, our own pair, passed as a system prompt. The prompts can be found in Table \ref{tab:contrastive_prompts}.

As for trained probes, we follow \citet{NEURIPS2025_cf42f133} and train six probes on base model instances of VEA. We label the base model's reasoning traces from eight benchmarks disjoint from our test sets with the judge of Section \ref{sec:setup}. Positives are the first sentence of a verbalization of evaluation-intent (EI) or test-question (TQ) awareness, and EA takes either as positive. Negatives are length- and format-matched sentences from traces containing no VEA. Activations are extracted from the token directly before each sentence. For each of EI, TQ, and EA we fit a mass-mean direction (MM) and a linear softmax classifier (SM), giving six probes: \textbf{EI-MM}, \textbf{EI-SM}, \textbf{TQ-MM}, \textbf{TQ-SM}, \textbf{EA-MM}, and \textbf{EA-SM}.

In order to fairly compare to the other methods, we choose which layer of the model to use to score the organism using held out judge samples. \sahar{is this heldout data on the base model? do we have results?} \evan{yes, they were supplied to me by Dan} For the contrastive means probes we use VEA \sahar{this is to test?} \evan{this is to select which layer probe to use} as the positive class and for the trained probes, we use their original target (e.g., EI or TQ). We select the highest performing layer, as measured by the AUC, per extraction site, meaning the same layer may not be selected at every point \sahar{at every point means for every probe?}.

\subsubsection{Jacobian Lens}

The Jacobian Lens maps a residual stream activation into vocabulary space by replacing the layers after layer $\ell$ with a first-order approximation of their effect, the Jacobian \citep{gurnee2026jlens}. This approximation is calculated as how a small perturbation of the activation at layer $\ell$ shifts the final layer residual stream, replacing the non-linear computations of subsequent layers with a linear map. To separate the model's general disposition to verbalize a token from the specific contextual disposition, the contribution is averaged over token positions and over many prompts. The Jacobian can then be applied in tandem with the unembedding matrix to visualize what tokens the activation is disposed to push the model toward.

\begin{equation}
    \text{lens}(h_{\ell}) = \text{softmax}\left( W_{U}\, \text{norm}(J_{\ell} h_{\ell}) \right).
\end{equation}

In order to test whether this approach can reliably predict the behavior of the model organism, we measured the AUC of how well the distributions of the probability mass of the buckets of tokens could separate this behavior. The buckets we used were Anth\_eval (taken from \citep{gurnee2026jlens}), Anth\_ctrl (recreation of the set from \citep{gurnee2026jlens}), min\_eval/deploy (of three sizes), and extended\_eval/deploy \daniel{do these need to be cited?}. The exact lists of the items in these buckets can be seen in Appendix \ref{app:token_buckets}. We combine these buckets in three ways: raw ($\text{Eval}$ or $\text{Deploy}$), control-subtracted ($\text{Eval} - \text{Control}$), and difference ($\text{Eval} - \text{Deploy}$). This yields 22 readouts, each scored as the bucket's log-probability mass, averaged over layers $\ell \in [24, 58]$. These layers are taken from the depth range in which \citet{gurnee2026jlens} locates the workspace (38-92\% of depth), mapped onto our 63 fitted lens layers, and are therefore fixed independently of our labels. We evaluate every readout at 11 extraction points across the input, reasoning, and output (Appendix \ref{app:extraction_points}).

\subsubsection{Activation Oracles}

Activation Oracles are a recently developed method that allows arbitrary questions to be asked about extracted activations from a model \citep{karvonen2026activation}. An oracle is specifically a copy of the base model that is trained with LoRA to perform various question-answering tasks given an extracted activation from the residual stream, which are passed into the first layer of the model (since they are of the same dimensions).

We use Activation Oracles to interrogate whether the model organism believes it is under evaluation or in deployment. To do so, we give the oracle an extracted activation from the oracle at one of three depths (25\%, 50\%, and 75\%) and a binary question. The question is \textit{Does the model believe it is in evaluation or in deployment?}, with or without a forcing prefix, \textit{Answer with 'evaluation' or 'deployment'.} that enforces the next token to either be \textit{evaluation} or \textit{deployment}. We collect the output from both orderings of \textit{evaluation} and \textit{deployment} to account for recency bias. We then compare the logit difference between \textit{evaluation} and \textit{deployment} as well as the mean of the two directions of questions.

==> tables/tab_gap1_probes_all10_two_sites.tex <==
\begin{table}[t]
\centering
\small
\caption{AUC for probe-based prediction of \emph{marker} emission for all ten probes, at \texttt{asst\_header} and the start of reasoning, under the X100 system prompt. Extends \Cref{tab:probes}. $^\dagger$: 95\% CI (Hanley--McNeil) includes 0.5. The last row of each block is the 95th percentile of the 12 neutral directions under the same layer selection.}
\label{tab:probes-all10-two-sites}
\begin{tabular}{l l rrrr r}
\toprule
Position & Probe & WildChat & BBH & EvalAwareBench & Triggers & Median \\
\midrule
\texttt{asst\_header} & TH-16 & 0.477$^\dagger$ & 0.931 & 0.595 & 0.443$^\dagger$ & 0.536 \\
 & TH-4 & 0.427 & 0.591 & 0.532 & 0.514$^\dagger$ & 0.523 \\
 & Anth & 0.399 & 0.658 & 0.454 & 0.452$^\dagger$ & 0.453 \\
 & E/NE & 0.448 & 0.317 & 0.554 & 0.459$^\dagger$ & 0.454 \\
 & EA-MM & 0.794 & 0.850 & 0.604 & 0.527$^\dagger$ & 0.699 \\
 & EA-SM & 0.806 & 0.684 & 0.512$^\dagger$ & 0.560$^\dagger$ & 0.622 \\
 & TQ-MM & 0.762 & 0.847 & 0.594 & 0.523$^\dagger$ & 0.678 \\
 & TQ-SM & 0.744 & 0.475$^\dagger$ & 0.584 & 0.478$^\dagger$ & 0.531 \\
 & EI-MM & 0.609 & 0.287 & 0.473$^\dagger$ & 0.429 & 0.451 \\
 & EI-SM & 0.709 & 0.284 & 0.475$^\dagger$ & 0.395 & 0.435 \\
 & \textit{neutral 95th pct} & 0.738 & 0.898 & 0.574 & 0.580 & 0.659 \\
\midrule
\texttt{think000} & TH-16 & 0.566 & 0.427 & 0.534 & 0.448$^\dagger$ & 0.491 \\
 & TH-4 & 0.623 & 0.479$^\dagger$ & 0.524$^\dagger$ & 0.463$^\dagger$ & 0.501 \\
 & Anth & 0.401 & 0.550 & 0.526$^\dagger$ & 0.434 & 0.480 \\
 & E/NE & 0.657 & 0.399 & 0.494$^\dagger$ & 0.478$^\dagger$ & 0.486 \\
 & EA-MM & 0.640 & 0.929 & 0.573 & 0.578 & 0.609 \\
 & EA-SM & 0.762 & 0.572 & 0.501$^\dagger$ & 0.604 & 0.588 \\
 & TQ-MM & 0.740 & 0.968 & 0.596 & 0.542$^\dagger$ & 0.668 \\
 & TQ-SM & 0.482$^\dagger$ & 0.829 & 0.531$^\dagger$ & 0.523$^\dagger$ & 0.527 \\
 & EI-MM & 0.437 & 0.153 & 0.506$^\dagger$ & 0.434 & 0.435 \\
 & EI-SM & 0.587 & 0.037 & 0.553 & 0.457$^\dagger$ & 0.505 \\
 & \textit{neutral 95th pct} & 0.729 & 0.951 & 0.539 & 0.499 & 0.634 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/tab_gap4_method_details.tex <==
\begin{table}[t]
\centering
\small
\caption{Setup of the three interpretability methods not given in the main text.}
\label{tab:method-details}
\begin{tabular}{l p{0.72\linewidth}}
\toprule
Setting & Value \\
\midrule
\multicolumn{2}{l}{\textit{Jacobian Lens}} \\
Lens & Published Neuronpedia lens for Qwen3.5-27B, fitted on the base model; not refitted on the organism \\
Fitting data & \texttt{wikitext-103-raw-v1} train; 1,000 prompts requested, 672 used before convergence ($\Delta < 0.002$); max sequence length 128; bfloat16 \\
Fit quality & Final identity distance 0.376 \\
Layers & 63 Jacobians (source layers 0--62, target layer 63); readouts averaged over layers 24--58 (38--92\% depth) \\
\midrule
\multicolumn{2}{l}{\textit{Activation Oracle}} \\
Checkpoint & Trained by us on Qwen3.5-27B with the released training code and recipe of \citet{karvonen2026activation}, unmodified \\
Training data & LatentQA, classification, and past-lens tasks (100k past-lens examples); activations injected from 25/50/75\% depth \\
Optimization & LoRA $r=64$, $\alpha=128$, dropout 0.05 on all attention and MLP projections; learning rate $10^{-5}$; 1 epoch; global batch 16; 4$\times$B200 \\
Readout layers & 16, 32, 48 (25/50/75\% depth) \\
\midrule
\multicolumn{2}{l}{\textit{Linear probes}} \\
Activations & Residual stream at the block input, base model for fitting and selection, organism for testing \\
Trained probes & Fitted at the token before each sentence; classes balanced by subsampling; softmax probe: 2-way softmax, SGD, lr 0.008, momentum 0.9, up to 300 epochs, following \citet{NEURIPS2025_cf42f133} \\
Nulls & 24 random and 12 neutral directions, put through the same per-position layer selection \\
\bottomrule
\end{tabular}
\end{table}


==> tables/tab_gap5_oracle_equal_selection.tex <==
\begin{table}[t]
\centering
\small
\caption{Activation Oracle against the same pipeline with the oracle adapter disabled, at \texttt{asst\_header} under the X100 system prompt. The first two columns reproduce \Cref{tab:oracle_benchmark} (the oracle's best readout, and that readout with the adapter off). The last column gives the adapter-off model the same choice among the 18 readouts (6 queries $\times$ 3 layers) that the oracle had: its best reaches the oracle's median AUC.}
\label{tab:oracle-equal-selection}
\begin{tabular}{l rrr}
\toprule
& Oracle & \multicolumn{2}{c}{Adapter disabled} \\
\cmidrule(lr){3-4}
Benchmark & unforced, avg, L48 & unforced, avg, L48 & forced, deploy first, L32 \\
\midrule
WildChat & 0.739 & 0.274 & 0.625 \\
BBH & 0.607 & 0.300 & 0.684 \\
EvalAwareBench & 0.576 & 0.551 & 0.560 \\
Triggers & 0.561 & 0.469 & 0.534 \\
\midrule
Median & 0.591 & 0.385 & 0.592 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/tab_gap5_selection_null.tex <==
\begin{table}[t]
\centering
\small
\caption{A null shared across methods. For each method we permute the \emph{marker} labels within each benchmark (2,000 permutations, one permutation applied to all of the method's readouts), recompute the median AUC across WildChat, BBH, EvalAwareBench and Triggers for each of its $K$ readouts, and take the maximum: the value a method with the same selection freedom reaches by chance. ``Best'' is the observed best median AUC under X100; ``All positions'' also maximizes over extraction positions (those with more than 30 rows per class on every benchmark). Every method exceeds its null ($p < 0.001$), so this null only rules out chance; the confounds of \Cref{sec:interp_results} are not addressed by it.}
\label{tab:selection-null}
\begin{tabular}{l r rrr rrr}
\toprule
& & \multicolumn{3}{c}{\texttt{asst\_header}} & \multicolumn{3}{c}{All positions} \\
\cmidrule(lr){3-5}\cmidrule(lr){6-8}
Method & $K$ & Best & Null 95\% & Null 99\% & Best & Null 95\% & Null 99\% \\
\midrule
Linear probes & 10 & 0.699 & 0.526 & 0.531 & 0.699 & 0.534 & 0.538 \\
Jacobian Lens & 22 & 0.667 & 0.526 & 0.532 & 0.667 & 0.535 & 0.539 \\
Activation Oracle & 18 & 0.591 & 0.527 & 0.532 & 0.670 & 0.535 & 0.539 \\
\quad adapter disabled & 18 & 0.592 & 0.528 & 0.533 & 0.592 & 0.535 & 0.539 \\
\bottomrule
\end{tabular}
\end{table}

